Active Learning with Label Comparisons

Supervised learning typically relies on manual annotation of the true labels. When there are many potential classes, searching for the best one can be prohibitive for a human annotator. On the other hand, comparing two candidate labels is often much easier. We focus on this type of pairwise supervision and ask how it can be used effectively in learning, and in particular in active learning. We obtain several insightful results in this context. In principle, finding the best of $k$ labels can be done with $k-1$ active queries. We show that there is a natural class where this approach is sub-optimal, and that there is a more comparison-efficient active learning scheme. A key element in our analysis is the "label neighborhood graph" of the true distribution, which has an edge between two classes if they share a decision boundary. We also show that in the PAC setting, pairwise comparisons cannot provide improved sample complexity in the worst case. We complement our theoretical results with experiments, clearly demonstrating the effect of the neighborhood graph on sample complexity.

==> draft_bits.tex <==
%% remark about equivalence of 1NN and H

Both our positive and negative results for $\H^{k,2}_{\linear}$ will employ the following equivalent parameterization of this class: $\set { h_{\cc}  : \quad \cc \in \R^k}$
where $\sbr{h_{\cc(x)}}_i = \|x - c_i \|_2$. 
Viewed this way, we refer to $c_i$ as the \emph{center} %\amirg{let's use US spelling: center. here and throughout.} 
of class $i$ and to the \emph{sorted order} of the classes as the order of the centers. For classes $i,j \in [k]$, define $\theta_{i,j}$
as the intersection of the lines $\set{w_i\cdot x + b_i : x \in \R}$ and $\set{w_j\cdot x + b_j : x \in \R}$. We use $\theta_i$ to denote $\theta_{i, i^-}$, where $i^-$ the class preceding $i$ in the total order, and the centers of the classes are chosen such that $\theta_i$ is the average between $c_{i^-}$ and $c_i$. Note that both $\set{c_i}_{i=1}^k$ and $\set{\theta_i}_{i=2}^k$
provide equivalent parameterization of the multi-class classifier;  See Figure \ref{fig:1nn} for an example with $k=3$ classes. 

